LLMEffiChecker: Understanding and Testing Efficiency Degradation of Large Language Models

In this paper, we make the first attempt to understand and test potential computation efficiency robustness in state-of-the-art LLMs. By analyzing the working mechanism and implementation of 20,543 public-accessible LLMs, we observe a fundamental property in LLMs that could be manipulated in an adversarial manner to reduce computation efficiency significantly. Our key motivation is to generate test inputs that could sufficiently delay the generation of EOS such that LLMs would have to go through enough iterations to satisfy the pre-configured threshold. We present \tool, which can work under both white-box setting and black-box setting. In the white-box scenario, \tool develops a gradient-guided technique that searches for a minimal and unnoticeable perturbation at character-level, token-level, and structure-level. In the black-box scenario, \tool employs a causal inference-based approach to find critical tokens and similarly applies three levels of imperceptible perturbation to them. Both the white-box and black-box settings effectively delay the appearance of EOS, compelling these inputs to reach the naturally-unreachable threshold. To demonstrate the effectiveness of \tool, we conduct a systematic evaluation on nine public-available LLMs: Google T5, AllenAI WMT14, Helsinki-NLP translator, Facebook FairSeq, UNICAMP-DL translator, MarianMT, Google FLAN-T5, MBZUAI LaMini-GPT and Salesforce CodeGen. Experimental results show that \tool can increase on average LLMs' response latency and energy consumption by 325\% to 3244\% and 344\% to 3616\%, respectively, by perturbing just one character or token in the input sentence.

==> Alg/alg.tex <==
% \begin{wrapfigure}{RT}{0.55\textwidth}
% \begin{minipage}{0.55\textwidth}
\begin{algorithm}[H]
\caption{\tool Attack} 
\label{alg:white}

\begin{flushleft}
 {\bf Input:} Seed input $x$, \\
{\bf Input:} NMT system under test $\mathcal{F}(\cdot)$, \\
{\bf Input:} Maximum perturbation $\epsilon$  \\
% \hspace*{0.02in} {\bf Input:}  A set of normal samples $\mathcal{X}_{normal}$   \\
% \hspace*{0.02in} {\bf Input:}  Given attack radius $r_2$ \\
 {\bf Output:} Test example $x'$\\
\end{flushleft}
\begin{algorithmic}[1]
\STATE $x' \Leftarrow x$ \xspace\xspace Initialize $x'$ with $x$
% \STATE $j \Leftarrow 0$ Initialize $j$ with 0


\WHILE{$||x' - x|| \le \epsilon$}
    \FOR{each $tk_i \in x'$}
        \STATE Compute $g_{i}$ according to \equref{eq:obj}
    \ENDFOR
    \STATE TK  $\Leftarrow Sort(tk_1, tk_2, \cdots, tk_m$) according to $g_{i}$
    % \STATE L $\Leftarrow$ Empty  List
    % \FOR{each $tk_i \in$ TK}
    \STATE $L  = $ GeneratePerturbation$(\text{TK}, x', \mathcal{F}(\cdot)$)
    % \STATE $L.add([tk_i, \delta])$
    % \ENDFOR
    \STATE $[tk, \Delta] =$ SelectBestPerturbation$(L, x', \mathcal{F}(\cdot))$
    \STATE $x' \Leftarrow$ replace $tk$ with $\Delta$ in $x'$
\ENDWHILE
\STATE return $x'$


\end{algorithmic}
\end{algorithm}
% \vspace{-3mm}
% \end{minipage}
% \end{wrapfigure}

==> Approach/attack_B.tex <==
\subsection{Detail Design}

\noindent\textbf{Finding Critical Tokens:} 
\textcolor{blue}{As we discussed in \secref{sec:background}, the computational efficiency of LLMs relies on the resultant output length for any given input. Based on the above conclusions and inspiration from \cite{jin2020bert}, our mechanism involves removing each token from the seed sentence. By comparing the output length of the modified sentence with the original output length, we pinpoint the sentence with the most substantial difference in output length from the seed sentence. Subsequently, we identify the missing token in this sentence, which constitute the critical tokens we are seeking.}

\textcolor{blue}{Formally, given a seed sentence $S_{\text{orig}} = [tk_{1}, tk_{2}, \cdots, tk_m]$, we generate a new sentence appearance $S_i$ by removing the token $tk_i$ from $S_{\text{orig}}$. Subsequently, we feed each $S_i$ and $S_{\text{orig}}$ into the target LLM to obtain the corresponding output lengths $O_i$ and $O$. Our objective is to identify the index $j$ that maximizes $\gamma_j$. Once this index $j$ is determined, the critical token is $tk_j$ in $S_{\text{orig}}$ (refer to Equation~\eqref{eq:b_obj}).
\begin{equation}
\label{eq:b_obj}
        \gamma_i = |O_i - O| \qquad  j = argmax_i\gamma_i  
\end{equation}
}





{\noindent\textbf{Input Mutation: }\textcolor{blue}{The character-level perturbations and structure-level perturbations described in }\secref{sec:whitebox}} \textcolor{blue}{are well-suited for black-box settings. Consequently, in \tool/B, we focus specifically on modifying token-level perturbations. Upon identification of the critical tokens, we proceed to randomly select tokens from the vocabulary to effect replacements.}


\noindent\textbf{Efficiency Degradation Detection:\TODO{delete or modify it?}}
After collecting candidate perturbations $L$, we select an optimal perturbation from the collected candidate sets.
Since our objective is searching this perturbation candidate set that will produce a longer output length, we straightforwardly test all perturbations in this set and select the optimal perturbation that produces the maximum output length.



==> Approach/overview_B.tex <==
\subsection{Design Overview}

\textcolor{blue}{\tool/B follows the design framework illustrated in \figref{fig:overview}. In contrast to \tool, the computation of gradients is unfeasible in the black-box scenario. An overview detailing the procedure for each iteration of \tool/B also contains three major steps:} 
\begin{enumerate}
%     \item  \textit{Finding critical tokens.} \textcolor{blue}{
%     For each seed sentence, we feed the seed sentence and all newly generated sentences into the model by deleting each word in the sentence one by one and record the output length. By analyzing the resulting output length list, we identify the sentence with the largest difference in output length from the seed sentence, and then determine the missing words in it, which are the critical tokens we are looking for.
% }
    \item  \textit{Finding critical tokens.} \textcolor{blue}{
    For each seed sentence, we find the critical tokens that have the highest impact on LLMs’ computation efficiency by measuring the prediction length change after deleting each token.
}


    \item  \textit{Mutating seed input sentences.} After identifying the critical tokens in the seed sentences, we mutate the seed sentences with three types of perturbations and generate three lists of similar sentences.

    \item \textit{Detecting efficiency degradation.} We feed the mutated sentences and the seed sentence into \textcolor{blue}{LLMs} and detect any efficiency degradation.
    
\end{enumerate}


==> Evaluation/detector.tex <==
% Table generated by Excel2LaTeX from sheet 'Detector'

\begin{table}[hbtp]
  \centering
  \caption{The accuracy and extra overheads of the detector}
  \resizebox{0.65\textwidth}{!}{
    \begin{tabular}{c|c|rrrr}
    \toprule[1.2pt]
    \multirow{2}[2]{*}{Subject} & \multirow{2}[2]{*}{Metric (\%)} & \multicolumn{4}{c}{Perturbation Type} \\
          &       & \multicolumn{1}{c}{\tool(C)} & \multicolumn{1}{c}{\tool(T)} & \multicolumn{1}{c}{\tool(S)} & \multicolumn{1}{c}{Mixed} \\
    \hline
    \multirow{4}[2]{*}{H-NLP} & Acc   & 99.98  & 99.99  & 99.98  & 99.98  \\
          & AUC   & 100.00  & 100.00  & 100.00  & 100.00  \\
          & Overheads & 0.17  & 0.32  & 0.18  & 0.74  \\
          & Energy & 0.09  & 0.17  & 0.12  & 0.48  \\
    \hline
    \multirow{4}[1]{*}{AllenAI} & Acc   & 100.00  & 100.00  & 87.00  & 98.00  \\
          & AUC   & 100.00  & 100.00  & 98.32  & 100.00  \\
          & Overheads & 0.17  & 0.08  & 0.49  & 0.86  \\
          & Energy & 0.11  & 0.05  & 0.30  & 0.79  \\
    \hline
    \multirow{4}[1]{*}{T5} & Acc   & 99.97  & 100.00  & 99.99  & 100.00  \\
          & AUC   & 100.00  & 100.00  & 100.00  & 100.00  \\
          & Overheads & 0.08  & 0.06  & 0.03  & 0.18  \\
          & Energy & 0.05  & 0.04  & 0.02  & 0.11  \\
    \bottomrule[1.2pt]
    \end{tabular}%
  }
  \label{tab:detector}%
\end{table}%


==> Evaluation/detector_B.tex <==
% Table generated by Excel2LaTeX from sheet 'Detector'

\begin{table}[hbtp]
  \centering
  \caption{The accuracy and extra overheads of the \tool-B detector}
  \resizebox{0.78\textwidth}{!}{
    \begin{tabular}{c|c|cccc}
    \toprule[1.2pt]
    \multirow{2}[2]{*}{\textbf{Subject}} & \multirow{2}[2]{*}{\textbf{Metric (\%)}} & \multicolumn{4}{c}{\textbf{Perturbation Type}} \\
          &       & \multicolumn{1}{c}{\textbf{\tool-B (C)}} & \multicolumn{1}{c}{\textbf{\tool-B (T)}} & \multicolumn{1}{c}{\textbf{\tool-B (S)}} & \multicolumn{1}{c}{\textbf{Mixed}} \\
    \hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{H-NLP}}} & \textbf{Acc} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.14  & 0.30  & 0.19  & 0.69 \\
      & \textbf{Energy} & 0.07  & 0.16  & 0.09  & 0.39 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{AllenAI}}} & \textbf{Acc} & 100.00 & 100.00 & 95.00 & 97.50 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.14  & 0.12  & 0.52  & 0.81 \\
      & \textbf{Energy} & 0.13  & 0.08  & 0.37  & 0.67 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{T5}}} & \textbf{Acc} & 100.00 & 100.00 & 97.50 & 97.50 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.06  & 0.08  & 0.03  & 0.17 \\
      & \textbf{Energy} & 0.04  & 0.04  & 0.03  & 0.12 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{U-DL}}} & \textbf{Acc} & 100.00 & 100.00 & 100.00 & 97.50 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.00  & 0.02  & 0.00  & 0.03 \\
      & \textbf{Energy} & 0.21  & 0.58  & 0.42  & 0.96 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{FairSeq}}} & \textbf{Acc} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.03  & 0.02  & 0.00  & 0.09 \\
      & \textbf{Energy} & 0.14  & 0.23  & 0.15  & 0.56 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{MarianMT}}} & \textbf{Acc} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.02  & 0.04  & 0.02  & 0.07 \\
      & \textbf{Energy} & 0.09  & 0.05  & 0.04  & 0.18 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{Flan-T5}}} & \textbf{Acc} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.07  & 0.12  & 0.05  & 0.17 \\
      & \textbf{Energy} & 0.07  & 0.09  & 0.04  & 0.29 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{LaMini-GPT}}} & \textbf{Acc} & 100.00 & 100.00 & 94.47 & 98.34 \\
      & \textbf{AUC} & 100.00 & 100.00 & 98.46 & 99.73 \\
      & \textbf{Overheads} & 0.03  & 0.06  & 0.05  & 0.08 \\
      & \textbf{Energy} & 0.05  & 0.32  & 0.18  & 0.53 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{CodeGen}}} & \textbf{Acc} & 100.00 & 100.00 & 99.87 & 99.98 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.15  & 0.42  & 0.29  & 0.84 \\
      & \textbf{Energy} & 0.12  & 0.45  & 0.20  & 0.86 \\
    \bottomrule[1.2pt]
    \end{tabular}%
  }
  \label{tab:detector_B}%
\end{table}%


==> Evaluation/new_detector.tex <==
% Table generated by Excel2LaTeX from sheet 'Detector'

\begin{table}[hbtp]
  \centering
  \caption{The accuracy and extra overheads of the \tool detector}
  \resizebox{0.78\textwidth}{!}{
    \begin{tabular}{c|c|cccc}
    \toprule[1.2pt]
    \multirow{2}[2]{*}{\textbf{Subject}} & \multirow{2}[2]{*}{\textbf{Metric (\%)}} & \multicolumn{4}{c}{\textbf{Perturbation Type}} \\
          &       & \multicolumn{1}{c}{\textbf{\tool(C)}} & \multicolumn{1}{c}{\textbf{\tool(T)}} & \multicolumn{1}{c}{\textbf{\tool(S)}} & \multicolumn{1}{c}{\textbf{Mixed}} \\
    \hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{H-NLP}}} & \textbf{Acc} & 99.98 & 99.99 & 99.98 & 99.98 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.17  & 0.32  & 0.18  & 0.74 \\
      & \textbf{Energy} & 0.09  & 0.17  & 0.12  & 0.48 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{AllenAI}}} & \textbf{Acc} & 100.00 & 100.00 & 87.00 & 98.00 \\
      & \textbf{AUC} & 100.00 & 100.00 & 98.32 & 100.00 \\
      & \textbf{Overheads} & 0.17  & 0.08  & 0.49  & 0.86 \\
      & \textbf{Energy} & 0.11  & 0.05  & 0.30  & 0.79 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{T5}}} & \textbf{Acc} & 99.97 & 100.00 & 99.99 & 100.00 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.08  & 0.06  & 0.03  & 0.18 \\
      & \textbf{Energy} & 0.05  & 0.04  & 0.02  & 0.11 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{U-DL}}} & \textbf{Acc} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.00  & 0.00  & 0.01  & 0.03 \\
      & \textbf{Energy} & 0.19  & 0.54  & 0.31  & 0.83 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{FairSeq}}} & \textbf{Acc} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.02  & 0.01  & 0.01  & 0.10 \\
      & \textbf{Energy} & 0.11  & 0.27  & 0.16  & 0.52 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{MarianMT}}} & \textbf{Acc} & 100.00 & 100.00 & 100.00 & 98.50 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.01  & 0.00  & 0.03  & 0.01 \\
      & \textbf{Energy} & 0.03  & 0.06  & 0.02  & 0.15 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{Flan-T5}}} & \textbf{Acc} & 83.65 & 91.00 & 90.50 & 92.66 \\
      & \textbf{AUC} & 89.42 & 91.38 & 93.98 & 97.38 \\
      & \textbf{Overheads} & 0.01  & 0.04  & 0.04  & 0.24 \\
      & \textbf{Energy} & 0.02  & 0.09  & 0.06  & 0.26 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{LaMini-GPT}}} & \textbf{Acc} & 100.00 & 100.00 & 92.50 & 99.00 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.00  & 0.01  & 0.01  & 0.05 \\
      & \textbf{Energy} & 0.06  & 0.25  & 0.14  & 0.47 \\
\hline
\multicolumn{1}{c|}{\multirow{4}[2]{*}{\textbf{CodeGen}}} & \textbf{Acc} & 100.00 & 100.00 & 98.47 & 100.00 \\
      & \textbf{AUC} & 100.00 & 100.00 & 100.00 & 100.00 \\
      & \textbf{Overheads} & 0.13  & 0.37  & 0.27  & 0.71 \\
      & \textbf{Energy} & 0.09  & 0.43  & 0.14  & 0.79 \\
    \bottomrule[1.2pt]
    \end{tabular}%
  }
  \label{tab:new_detector}%
\end{table}%


==> Table/c_black.tex <==
% Table generated by Excel2LaTeX from sheet 'transfer'
\begin{table}[htbp]
  \centering
  \caption{The maximum I-FLOPs of blackbox character-level attack}
  \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{c|c|rrrrr}
    \toprule
    \textbf{Source} & \textbf{Target } & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{2}} & \multicolumn{1}{c}{\textbf{3}} & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{5}} \\
    \midrule
    \multirow{2}[1]{*}{\textbf{H-NLP}} & \textbf{FairSeq} & 900.00  & 273.08  & 2400.00  & 573.08  & 2400.00  \\
          & \textbf{T5} & 1700.00  & 1700.00  & 1700.00  & 1700.00  & 1700.00  \\
    \midrule
    \multirow{2}[2]{*}{\textbf{FairSeq}} & \textbf{H-NLP} & 250.00  & 325.00  & 400.00  & 400.00  & 433.33  \\
          & \textbf{T5} & 1400.00  & 1400.00  & 1400.00  & 1400.00  & 1400.00  \\
    \midrule
    \multirow{2}[2]{*}{\textbf{T5}} & \textbf{H-NLP} & 3733.33  & 3733.33  & 3733.33  & 3733.33  & 3733.33  \\
          & \textbf{FairSeq} & 1177.78  & 1337.50  & 1542.86  & 1337.50  & 1337.50  \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:c_black}%
\end{table}%


==> Table/case.tex <==
% Table generated by Excel2LaTeX from sheet 'case'

\vspace*{\fill}
 \begin{CJK}{UTF8}{gbsn}
\begin{table}[htbp]
  \centering
  \caption{The benign and adversarial examples under different settings}
  \resizebox{1.02\linewidth}{!}{
    \begin{tabular}{|c|c|l|l|}
    \toprule
    \multicolumn{1}{|l|}{\textbf{Attack Type}} & \textbf{NMT } & \textbf{Benign} & \textbf{Adversarial 1} \\
    \midrule
    \multirow{9}[18]{*}{\textbf{Token}} & \multirow{3}[6]{*}{\textbf{H-NLP}} & Let me see. & 哎 me see \\
\cmidrule{3-4}          &       & I am here. & I▁am going. \\
\cmidrule{3-4}          &       & He is back. & He is 视 \\
\cmidrule{2-4}          & \multirow{3}[6]{*}{\textbf{FairSeq}} & configure, verify, and troubleshoot vtp & configure, bebelus, and troubleshoot vtp \\
\cmidrule{3-4}          &       & finger-pointing politicians and chest-beating nationalists  & classmates-pointing politicians and chest-beating nationalists \\
\cmidrule{3-4}          &       & in the two nations will make rational discussion nearly impossible &  in the two nations will make rational discussion nearly impossible. \\
\cmidrule{2-4}          & \multirow{3}[6]{*}{\textbf{T5}} & The Commission's report sets out a detailed analysis of all the replies. & The Commission's report sets out a detailed analysis of all the replies Gefahr \\
\cmidrule{3-4}          &       & The October European Council meeting will return to the issue of migration. & The October European Council meeting will return to the issue of migration not \\
\cmidrule{3-4}          &       & on z/os the maximum length of the attribute is 256 bytes. on all other platforms it is 1024 bytes. & on z presenceos the maximum length of the attribute is 256 bytes. on all other platforms it is 1024 bytes. \\
    \midrule
    \multirow{9}[18]{*}{\textbf{Character}} & \multirow{3}[6]{*}{\textbf{H-NLP}} & You have heart disease. & You have heart Odisease. \\
\cmidrule{3-4}          &       & This is my question. & ThWis is my question. \\
\cmidrule{3-4}          &       & I'm a little confused. & I'm a litt\$le confused. \\
\cmidrule{2-4}          & \multirow{3}[6]{*}{\textbf{FairSeq}} & President Juncker: ‘Europe needs a genuine security union'  & President Juncker: ‘Europe needs a genuine security uni(on' " \\
\cmidrule{3-4}          &       & step up the cooperation on return and readmission. & step up the cooperation on return and readmis0sion. \\
\cmidrule{3-4}          &       & In the refugee crisis, Turkey and the EU walk together and work together. & In Ythe refugee crisis, Turkey and Ythe EU walk togeYther and work togeYther. \\
\cmidrule{2-4}          & \multirow{3}[6]{*}{\textbf{T5}} & load, performance, or scalability & load, perf"ormance, "or scalability \\
\cmidrule{3-4}          &       & will hell swallow you up? & will hell swallow \$you up? \\
\cmidrule{3-4}          &       & shengli oilfield used euronavy es301 to make coatings to offshore tidal zone. & shengli oil[field used euronavy es301 to make coatings to offshore tidal zone. \\
    \bottomrule
    \end{tabular}%
    }
    \label{tab:a_case}%
\end{table}%
 \end{CJK}
\vspace*{\fill}

==> Table/character.tex <==
% Table generated by Excel2LaTeX from sheet 'character'
\begin{table}[htbp]
  \centering
  \caption{The severity of character-level adversarial attacks}
  \resizebox{.49\textwidth}{!}{
        \begin{tabular}{c|c|cc|cc|cc}
    \toprule
    \multirow{2}[2]{*}{\textbf{NMT}} & \multirow{2}[2]{*}{\textbf{Perturbation}} & \multicolumn{2}{c|}{\textbf{I-FLOPs}} & \multicolumn{2}{c|}{\textbf{I-Latency    (CPU)}} & \multicolumn{2}{c}{\textbf{I-Latency    (GPU)}} \\
          &       & \textbf{Baseline} & \textbf{Ours} & \textbf{Baseline} & \textbf{Ours} & \textbf{Baseline} & \textbf{Ours} \\
    \midrule
    \multirow{5}[2]{*}{\textbf{H-NLP}} & \textbf{1} & 20.09  & \textbf{389.36 } & 21.27  & \textbf{431.72 } & 11.84  & \textbf{368.08 } \\
          & \textbf{2} & 20.09  & \textbf{879.16 } & 21.29  & \textbf{978.47 } & 12.07  & \textbf{840.47 } \\
          & \textbf{3} & 20.09  & \textbf{1102.86 } & 21.29  & \textbf{1232.71 } & 12.07  & \textbf{1056.88 } \\
          & \textbf{4} & 20.09  & \textbf{1189.48 } & 21.29  & \textbf{1328.29 } & 12.07  & \textbf{1136.70 } \\
          & \textbf{5} & 20.09  & \textbf{1224.91 } & 21.29  & \textbf{1366.22 } & 12.07  & \textbf{1174.57 } \\
    \midrule
    \multirow{5}[2]{*}{\textbf{FairSeq}} & \textbf{1} & 0.28  & \textbf{36.23 } & 0.71  & \textbf{38.59 } & 3.15  & \textbf{40.13 } \\
          & \textbf{2} & 0.28  & \textbf{87.92 } & 0.71  & \textbf{97.37 } & 3.17  & \textbf{94.31 } \\
          & \textbf{3} & 0.28  & \textbf{145.60 } & 0.71  & \textbf{164.90 } & 3.17  & \textbf{155.43 } \\
          & \textbf{4} & 0.28  & \textbf{190.43 } & 0.71  & \textbf{217.94 } & 3.17  & \textbf{204.02 } \\
          & \textbf{5} & 0.28  & \textbf{223.07 } & 0.71  & \textbf{255.42 } & 3.17  & \textbf{235.93 } \\
    \midrule
    \multirow{5}[2]{*}{\textbf{T5}} & \textbf{1} & 5.60  & \textbf{217.46 } & 6.39  & \textbf{249.44 } & 5.71  & \textbf{229.70 } \\
          & \textbf{2} & 5.56  & \textbf{249.88 } & 6.37  & \textbf{286.81 } & 5.69  & \textbf{258.35 } \\
          & \textbf{3} & 5.56  & \textbf{267.58 } & 6.37  & \textbf{307.57 } & 5.69  & \textbf{273.41 } \\
          & \textbf{4} & 5.56  & \textbf{276.33 } & 6.37  & \textbf{318.40 } & 5.69  & \textbf{283.37 } \\
          & \textbf{5} & 5.56  & \textbf{280.10 } & 6.37  & \textbf{323.67 } & 5.69  & \textbf{286.84 } \\
    \bottomrule
    \end{tabular}%
   }
  \label{tab:character_res}%
\end{table}%


==> Table/model.tex <==
% Table generated by Excel2LaTeX from sheet 'models'
\begin{table}[tbp]
  \centering
  \caption{The NMT systems under test in our experiments}
  \resizebox{0.65\textwidth}{!}{
    \begin{tabular}{c|cccc}
    \toprule
    Model  & Source & Target & Vocab Size &  \texttt{max\_length} \\
    \midrule
    H-NLP & En    & De    & 65,001        & 512 \\
    AllenAi  & En    & De    & 42,024      & 200 \\
    T5    & En    & Zh    & 32,100    & 200 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:model}%
   \vspace{-2mm}
\end{table}%


==> Table/new_severity.tex <==
% Table generated by Excel2LaTeX from sheet 'Effectiveness'
% Table generated by Excel2LaTeX from sheet 'Effectiveness'
\begin{table*}[tp]
  \centering
  \caption{The Effectiveness Results of \textcolor{blue}{\tool} in Degrading \textcolor{blue}{LLMs} Performance}
  \resizebox{0.98\textwidth}{!}{
        \begin{tabular}{c|c|rrr|rrr|rrr|rrr|rrr}
    \toprule[1.2pt]
    \multirow{2}[2]{*}{\textbf{Subject}} & \multirow{2}[2]{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{I-Loops}} & \multicolumn{3}{c|}{\textbf{I-Latency(CPU)}} & \multicolumn{3}{c|}{\textbf{I-Energy(CPU)}} & \multicolumn{3}{c|}{\textbf{I-Latency(GPU)}} & \multicolumn{3}{c}{\textbf{I-Energy(GPU)}} \\
          &       & \multicolumn{1}{c}{\textbf{$\epsilon$ = 1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =3 }} \\
\midrule
\multirow{7}[3]{*}{\textbf{H-NLP}} & \textbf{\textbf{Seq2Sick}} & 4.31  & 5.84  & 12.28 & 4.83  & 8.85  & 19.55 & 4.84  & 8.85  & 21.47 & 3.73  & 5.90  & 13.24 & 3.77  & 5.96  & 13.33 \\
      & \textbf{SynError} & 19.09 & 19.59 & 19.59 & 19.35 & 19.82 & 19.82 & 19.63 & 20.10 & 20.10 & 14.14 & 14.52 & 14.52 & 14.27 & 14.65 & 14.65 \\
      & \textbf{SIT}   & 11.83 & 5.99  & 5.35  & -1.68 & -8.53 & -11.21 & 8.17  & 6.32  & 7.41  & 9.84  & 5.50  & 5.75  & 9.90  & 5.58  & 5.83 \\
      & \textbf{TransRepair} & 0.17  & 0.17  & 0.17  & 0.76  & 0.10  & 0.10  & 0.93  & 0.33  & 0.33  & -0.07 & 0.00  & 0.00  & -0.07 & 0.00  & 0.00 \\
      & \textbf{\tool(C)} & 564.45 & 995.45 & 1357.77 & 764.92 & 1487.92 & 2015.70 & 785.60 & 1471.26 & 1967.05 & 462.24 & 851.80 & 1116.80 & 406.39 & 755.18 & 972.92 \\
      & \textbf{\tool(T)} & 2697.77 & 3735.38 & 3917.91 & 3153.97 & 4481.93 & 4681.28 & 3052.62 & 4544.65 & 4759.71 & 1953.57 & 2729.83 & 2854.89 & 1532.91 & 2137.53 & 2221.66 \\
      & \textbf{\tool(S)} & 142.31 & 311.06 & 612.08 & 146.51 & 451.93 & 877.79 & 147.70 & 461.30 & 870.72 & 101.21 & 275.58 & 523.04 & 95.05 & 259.88 & 508.80 \\
\midrule
\multirow{7}[3]{*}{\textbf{AllenAI}} & \textbf{Seq2Sick} & 1.72  & 2.22  & 2.15  & 1.48  & 2.06  & 1.35  & 1.19  & 1.76  & 1.10  & 1.57  & 1.41  & 0.38  & 1.70  & 1.57  & 0.57 \\
      & \textbf{SynError} & 0.38  & 0.38  & 0.38  & 1.89  & 1.89  & 1.89  & 1.75  & 1.75  & 1.75  & -0.85 & -0.85 & -0.85 & -0.71 & -0.71 & -0.71 \\
      & \textbf{SIT}   & 7.06  & 4.12  & 6.67  & 1.73  & -3.24 & -4.64 & 1.73  & -3.24 & -4.60 & 3.95  & 14.25 & -2.05 & 4.12  & 14.64 & -1.60 \\
      & \textbf{TransRepair} & 0.08  & 0.08  & 0.08  & -0.37 & -0.37 & -0.37 & -0.55 & -0.55 & -0.55 & -0.15 & -0.15 & -0.15 & -0.14 & -0.14 & -0.14 \\
      & \textbf{\tool(C)} & 35.16 & 74.90 & 103.36 & 26.69 & 45.77 & 85.09 & 27.48 & 48.09 & 86.00 & 21.82 & 35.43 & 91.48 & 22.12 & 43.21 & 98.46 \\
      & \textbf{\tool(T)} & 24.83 & 42.04 & 56.75 & 49.12 & 62.84 & 67.98 & 49.99 & 62.65 & 69.06 & 30.65 & 41.32 & 46.09 & 31.00 & 41.81 & 49.66 \\
      & \textbf{\tool(S)} & 66.21 & 108.67 & 128.60 & 86.05 & 139.03 & 164.57 & 84.17 & 135.71 & 160.95 & 69.57 & 112.88 & 132.68 & 68.79 & 115.23 & 137.06 \\
\midrule
\multirow{7}[3]{*}{\textbf{T5}} & \textbf{Seq2Sick} & 7.09  & 6.28  & -6.03 & 7.21  & 6.04  & -5.97 & 8.55  & 6.88  & -5.16 & 9.01  & 8.00  & -3.97 & 8.85  & 16.94 & 4.50 \\
      & \textbf{SynError} & 2.18  & 2.18  & 2.18  & 3.20  & 3.20  & 3.20  & 2.11  & 2.11  & 2.11  & 1.02  & 1.02  & 1.02  & 1.13  & 1.13  & 1.13 \\
      & \textbf{SIT}   & -8.06 & 1.05  & 6.27  & -4.51 & 7.79  & 7.38  & -3.79 & 9.84  & 10.59 & -10.99 & 3.57  & 7.74  & -10.90 & 3.78  & 8.07 \\
      & \textbf{TransRepair} & 3.73  & 8.06  & 8.06  & 4.90  & 9.47  & 9.26  & 6.42  & 11.39 & 10.74 & 3.70  & 8.34  & 8.35  & 3.76  & 8.42  & 8.39 \\
      & \textbf{\tool(C)} & 168.92 & 198.36 & 205.37 & 191.05 & 225.48 & 233.01 & 194.45 & 228.02 & 234.04 & 164.61 & 194.79 & 202.28 & 165.38 & 195.77 & 203.29 \\
      & \textbf{\tool(T)} & 307.27 & 328.94 & 328.94 & 352.14 & 376.55 & 376.55 & 347.74 & 373.85 & 373.85 & 305.37 & 325.61 & 325.61 & 331.85 & 352.25 & 352.25 \\
      & \textbf{\tool(S)} & 77.67 & 80.56 & 82.52 & 85.72 & 89.11 & 91.38 & 86.90 & 90.29 & 92.56 & 75.77 & 78.68 & 80.66 & 68.79 & 73.03 & 74.56 \\
\midrule
\multirow{7}[3]{*}{\textbf{U-DL}} & \textbf{Seq2Sick} & 0.59  & 1.22  & 2.71  & -0.30 & 0.97  & 2.47  & 2.70  & 4.07  & 5.80  & 0.96  & 1.72  & 3.17  & 0.98  & 1.74  & 3.20 \\
      & \textbf{SynError} & 0.02  & 0.02  & 0.02  & -0.97 & -0.97 & -0.97 & 2.01  & 2.01  & 2.01  & -0.25 & -0.25 & -0.25 & -0.24 & -0.24 & -0.24 \\
      & \textbf{SIT}   & 16.73 & 6.40  & 4.26  & 15.50 & 4.15  & 2.45  & 18.90 & 9.37  & 7.56  & 17.16 & 6.30  & 4.81  & 17.18 & 6.33  & 4.82 \\
      & \textbf{TransRepair} & 11.36 & 10.66 & 10.82 & 7.53  & 7.09  & 7.09  & 10.07 & 9.94  & 9.95  & 11.46 & 11.45 & 11.59 & 11.43 & 11.41 & 11.55 \\
      & \textbf{\tool(C)} & 258.07 & 390.60 & 469.24 & 261.02 & 405.80 & 494.30 & 288.15 & 439.72 & 532.81 & 253.46 & 383.78 & 461.51 & 253.45 & 383.82 & 461.64 \\
      & \textbf{\tool(T)} & 604.17 & 642.38 & 642.38 & 655.13 & 696.56 & 696.56 & 697.90 & 741.86 & 741.86 & 595.88 & 634.44 & 634.44 & 596.49 & 635.08 & 635.08 \\
      & \textbf{\tool(S)} & 406.92 & 592.52 & 702.89 & 438.23 & 632.64 & 753.88 & 465.04 & 673.76 & 800.25 & 404.42 & 583.65 & 694.40 & 401.74 & 583.99 & 694.84 \\
\midrule
\multirow{7}[3]{*}{\textbf{FairSeq}} & \textbf{Seq2Sick} & 0.61  & 0.64  & -1.33 & 0.46  & -0.75 & -1.48 & 3.60  & 2.91  & 2.04  & 0.05  & 0.15  & -1.25 & 0.08  & 0.20  & -1.20 \\
      & \textbf{SynError} & 0.25  & 0.25  & 0.25  & -2.67 & -2.57 & -2.57 & -0.06 & 0.03  & 0.03  & 0.07  & 0.07  & 0.07  & 0.08  & 0.08  & 0.08 \\
      & \textbf{SIT}   & -1.15 & -2.15 & -1.56 & -4.46 & -7.26 & -6.73 & 0.13  & -1.90 & -1.63 & -2.34 & -1.51 & -2.37 & -2.37 & -1.52 & -2.37 \\
      & \textbf{TransRepair} & 0.26  & 0.25  & 0.25  & 0.02  & 0.01  & 0.05  & 0.67  & 0.66  & 0.69  & -0.03 & -0.01 & -0.01 & -0.03 & 0.00  & 0.00 \\
      & \textbf{\tool(C)} & 22.53 & 37.68 & 59.26 & 15.87 & 29.07 & 49.18 & 20.47 & 34.62 & 55.44 & 18.07 & 31.53 & 51.79 & 18.08 & 31.55 & 51.85 \\
      & \textbf{\tool(T)} & 33.73 & 62.13 & 76.41 & 23.97 & 55.26 & 70.28 & 29.79 & 63.19 & 79.41 & 28.62 & 59.42 & 75.47 & 28.60 & 59.42 & 75.47 \\
      & \textbf{\tool(S)} & 19.42 & 30.87 & 37.82 & 14.01 & 23.67 & 31.31 & 18.23 & 28.59 & 36.73 & 14.84 & 24.87 & 31.68 & 14.86 & 24.91 & 31.72 \\
\midrule
\multirow{7}[3]{*}{\textbf{MarianMT}} & \textbf{Seq2Sick} & -0.06 & -1.78 & -6.61 & -2.69 & -4.85 & -9.87 & 2.07  & 0.05  & -4.26 & 1.12  & -1.24 & -4.58 & 1.09  & -1.26 & -4.60 \\
      & \textbf{SynError} & 3.00  & 3.66  & 3.62  & 1.09  & 1.31  & 1.15  & 3.75  & 4.12  & 3.95  & 1.78  & 2.30  & 2.13  & 1.75  & 2.27  & 2.12 \\
      & \textbf{SIT}   & 1.94  & -0.27 & -0.82 & -1.91 & -3.95 & -5.03 & 3.95  & 2.00  & 0.71  & 1.23  & -0.59 & -1.64 & 1.20  & -0.59 & -1.62 \\
      & \textbf{TransRepair} & 0.03  & 0.95  & 0.68  & -0.89 & -0.65 & -1.06 & 1.50  & 1.77  & 1.36  & 0.06  & 0.24  & -0.02 & 0.05  & 0.23  & -0.03 \\
      & \textbf{\tool(C)} & 54.10 & 113.20 & 222.04 & 41.58 & 102.38 & 226.68 & 51.56 & 119.53 & 274.26 & 52.98 & 113.90 & 210.12 & 52.89 & 113.88 & 210.12 \\
      & \textbf{\tool(T)} & 231.65 & 550.07 & 726.61 & 234.93 & 564.34 & 770.28 & 269.58 & 660.70 & 893.87 & 223.56 & 544.49 & 728.90 & 223.48 & 544.28 & 728.68 \\
      & \textbf{\tool(S)} & 42.77 & 72.19 & 89.17 & 33.89 & 72.33 & 90.33 & 40.27 & 84.89 & 106.84 & 41.21 & 77.28 & 95.68 & 41.19 & 77.21 & 95.61 \\
\midrule
\multirow{7}[3]{*}{\textbf{Flan-T5}} & \textbf{Seq2Sick} & 6.64  & 10.31 & 13.09 & 5.97  & 9.68  & 11.76 & 14.05 & 18.79 & 22.16 & 5.76  & 9.35  & 11.96 & 5.74  & 9.34  & 11.92 \\
      & \textbf{SynError} & 0.05  & 0.05  & 0.05  & -1.73 & -1.73 & -1.73 & 6.02  & 6.02  & 6.02  & 5.62  & 5.62  & 5.62  & -7.51 & -7.51 & -7.51 \\
      & \textbf{SIT}   & 87.52 & 43.57 & 42.95 & 86.40 & 40.87 & 40.36 & 85.17 & 59.87 & 55.88 & 82.96 & 43.18 & 44.38 & 83.07 & 43.33 & 44.51 \\
      & \textbf{TransRepair} & -1.48 & -1.77 & -1.48 & -1.32 & -1.73 & -1.32 & 1.99  & 1.44  & 1.84  & -1.47 & -1.81 & -1.51 & -1.54 & -1.87 & -1.56 \\
      & \textbf{\tool(C)} & 327.55 & 566.82 & 625.69 & 329.99 & 564.27 & 621.78 & 381.37 & 647.48 & 715.92 & 333.91 & 574.26 & 634.28 & 334.03 & 574.53 & 634.51 \\
      & \textbf{\tool(T)} & 1209.50 & 1306.26 & 1349.04 & 1229.54 & 1327.42 & 1372.96 & 1409.23 & 1524.04 & 1578.49 & 1227.99 & 1325.01 & 1368.67 & 1229.06 & 1326.23 & 1369.93 \\
      & \textbf{\tool(S)} & 554.58 & 937.63 & 1063.39 & 552.96 & 952.73 & 1087.15 & 637.50 & 1094.72 & 1253.29 & 564.39 & 948.81 & 1076.25 & 564.90 & 949.32 & 1076.86 \\
\midrule
\multirow{7}[3]{*}{\textbf{LaMini-GPT}} & \textbf{Seq2Sick} & 21.91 & 21.81 & 15.24 & 121.46 & 121.66 & 88.75 & 140.43 & 140.48 & 101.57 & 98.56 & 97.73 & 69.70 & 98.85 & 98.03 & 69.97 \\
      & \textbf{SynError} & 87.81 & 88.68 & 96.68 & 377.07 & 403.58 & 429.18 & 438.06 & 468.04 & 498.53 & 318.71 & 333.48 & 354.60 & 319.06 & 333.86 & 355.09 \\
      & \textbf{SIT}   & 153.80 & 152.34 & 137.53 & 867.02 & 916.92 & 747.65 & 1,014.25 & 1,069.92 & 870.79 & 659.99 & 651.73 & 552.49 & 660.31 & 652.99 & 553.72 \\
      & \textbf{TransRepair} & 29.39 & 26.51 & 26.74 & 144.03 & 140.82 & 140.73 & 168.75 & 163.40 & 164.34 & 130.07 & 119.77 & 130.57 & 130.42 & 120.23 & 131.11 \\
      & \textbf{\tool(C)} & 323.34 & 367.46 & 376.55 & 2091.80 & 2643.98 & 2707.52 & 2403.58 & 3098.30 & 3169.53 & 1598.12 & 1997.75 & 2043.54 & 1597.50 & 1995.33 & 2041.12 \\
      & \textbf{\tool(T)} & 368.67 & 379.73 & 379.73 & 2539.10 & 2588.35 & 2588.35 & 3066.39 & 3130.40 & 3130.40 & 2106.89 & 2148.49 & 2148.49 & 2104.61 & 2146.16 & 2146.16 \\
      & \textbf{\tool(S)} & 347.41 & 366.07 & 366.42 & 2157.36 & 2371.21 & 2372.00 & 2510.74 & 2792.73 & 2793.60 & 1746.59 & 1919.43 & 1920.28 & 1747.96 & 1919.32 & 1920.17 \\
\midrule
\multirow{7}[3]{*}{\textbf{CodeGen}} & \textbf{Seq2Sick} & 5.10  & 5.10  & 5.10  & 13.34 & 13.34 & 13.34 & 16.68 & 16.68 & 16.68 & 17.06 & 17.06 & 17.06 & 17.10 & 17.10 & 17.10 \\
      & \textbf{SynError} & 26.48 & 26.49 & 27.54 & 83.33 & 83.26 & 85.38 & 89.39 & 89.34 & 91.54 & 87.61 & 87.54 & 89.78 & 87.65 & 87.58 & 89.81 \\
      & \textbf{SIT}   & 54.06 & 41.45 & 44.71 & 202.97 & 145.02 & 158.70 & 213.45 & 153.11 & 168.58 & 223.83 & 161.93 & 181.19 & 223.90 & 162.00 & 181.28 \\
      & \textbf{TransRepair} & 77.64 & 80.47 & 80.84 & 286.84 & 294.79 & 294.88 & 296.86 & 308.83 & 309.09 & 309.52 & 330.97 & 333.95 & 309.68 & 331.24 & 334.22 \\
      & \textbf{\tool(C)} & 109.93 & 139.88 & 168.23 & 321.08 & 434.06 & 533.72 & 336.01 & 453.64 & 558.45 & 351.20 & 478..08 & 592.39 & 351.46 & 478.36 & 592.75 \\
      & \textbf{\tool(T)} & 182.42 & 182.42 & 182.42 & 578.30 & 578.30 & 578.30 & 602.68 & 602.68 & 602.68 & 639.91 & 639.91 & 639.91 & 640.26 & 640.26 & 640.26 \\
      & \textbf{\tool(S)} & 176.30 & 187.59 & 187.59 & 575.42 & 615.61 & 615.61 & 593.11 & 635.62 & 635.62 & 607.64 & 653.51 & 653.51 & 607.97 & 653.91 & 653.91 \\
    \bottomrule[1.2pt]
    \end{tabular}%
    }
  \label{tab:new_severity}%
\end{table*}%



==> Table/nmt_table.tex <==
% Table generated by Excel2LaTeX from sheet 'NMTStudy'

\begin{table}[tbp]
  \centering  

  \caption{Top 10 popular NMT systems on HuggingFace website (the order is based on the number of downloads)\TODO{text generation}}
  \resizebox{0.65\textwidth}{!}{
      \begin{tabular}{c|lcc}
    \toprule
    \textbf{Rank} & \multicolumn{1}{c}{\textbf{Model Name }} & \textbf{max\_length} & \textbf{\# of Downloads} \\
    \midrule
    \textbf{1} & Helsinki-NLP/opus-mt-zh-en & 512   & 3141840 \\
    \textbf{2} & Google/t5-base & 300   & 1736544 \\
    \textbf{3} & Helsinki-NLP/opus-mt-en-de & 512   & 749228 \\
    \textbf{4} & Helsinki-NLP/opus-mt-en-ROMANCE & 512   & 599267 \\
    \textbf{5} & Google/t5-small & 300   & 592793 \\
    \textbf{6} & Helsinki-NLP/opus-mt-ar-en & 512   & 196033 \\
    \textbf{7} & Helsinki-NLP/opus-mt-de-en & 512   & 129923 \\
    \textbf{8} & Helsinki-NLP/opus-mt-es-en & 512   & 111028 \\
    \textbf{9} & Helsinki-NLP/opus-mt-ROMANCE-en & 512   & 92987 \\
    \textbf{10} & Helsinki-NLP/opus-mt-fr-en & 512   & 91552 \\
    % \textbf{11} & Google/t5-large & 300   & 86685 \\
    % \textbf{12} & facebook/mbart-large-en-ro & 1024  & 60718 \\
    % \textbf{13} & Helsinki-NLP/opus-mt-ru-en & 512   & 57630 \\
    % \textbf{14} & facebook/mbart-large-cc25 & 1024  & 54778 \\
    % \textbf{15} & Google/t5-3b & 300   & 38587 \\
    \bottomrule
    \end{tabular}%
  \label{tab:nmt}%
  \vspace{-8mm}
  }
\end{table}%


==> Table/overheads.tex <==


% Table generated by Excel2LaTeX from sheet 'Overheads'
\begin{table}[htbp]
  \centering
  \caption{Average overheads of \tool (s)}
  \resizebox{0.65\textwidth}{!}{
        \begin{tabular}{c|c|rrr|r}
    \toprule[1.2pt]
    Method & $\epsilon$    & \multicolumn{1}{c}{H-NLP} & \multicolumn{1}{c}{AllenAI} & \multicolumn{1}{c|}{T5} & \multicolumn{1}{c}{Average} \\
    \hline
    \multirow{3}[2]{*}{\tool(C)} & 1     & 11.40  & 21.14  & 18.50  & 17.01  \\
          & 2     & 31.80  & 44.66  & 45.59  & 40.68  \\
          & 3     & 59.76  & 69.56  & 74.48  & 67.93  \\
    \hline
    \multirow{3}[2]{*}{\tool(T)} & 1     & 7.50  & 18.45  & 22.62  & 16.19  \\
          & 2     & 31.41  & 39.48  & 61.86  & 44.25  \\
          & 3     & 62.50  & 62.54  & 100.01  & 75.02  \\
    \hline
    \multirow{3}[2]{*}{\tool(S)} & 1     & 10.52  & 39.19  & 6.73  & 18.81  \\
          & 2     & 23.33  & 75.21  & 17.45  & 38.66  \\
          & 3     & 38.93  & 106.35  & 27.71  & 57.66  \\
    \bottomrule[1.2pt]
    \end{tabular}%
    }
  \label{tab:overheads}%
\end{table}%


==> Table/senstive.tex <==
% Table generated by Excel2LaTeX from sheet 'senstive'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
  \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{c|c|ccccc}
    \toprule
    Method & Subject & 1     & 2     & 3     & 4     & 5 \\
    \midrule
    \multirow{9}[4]{*}{C} & \multirow{3}[2]{*}{H-NLP} & 140.82  & 178.22  & 244.15  & 438.28  & 384.41  \\
          &       & 324.37  & 416.10  & 603.46  & 1078.07  & 924.46  \\
          &       & 401.73  & 576.18  & 785.23  & 1449.32  & 1253.13  \\ \cline{2-7}
& \multirow{3}[1]{*}{FairSeq} & 16.64  & 19.47  & 21.43  & 23.60  & 25.66  \\
          &       & 29.95  & 33.40  & 39.09  & 42.11  & 47.71  \\
          &       & 44.83  & 51.60  & 55.61  & 60.70  & 69.43  \\ \cline{2-7}
          & \multirow{3}[1]{*}{T5} & 209.39  & 41.62  & 30.39  & 25.63  & 29.02  \\
          &       & 244.97  & 52.92  & 38.90  & 33.12  & 36.84  \\
          &       & 266.72  & 60.37  & 45.26  & 39.26  & 42.38  \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:addlabel}%
\end{table}%


==> Table/severity.tex <==
% Table generated by Excel2LaTeX from sheet 'Effectiveness'
% Table generated by Excel2LaTeX from sheet 'Effectiveness'
\begin{table*}[tp]
  \centering
  \caption{The Effectiveness Results of Test Samples in Degrading NMT Performance}
  \resizebox{0.98\textwidth}{!}{
        \begin{tabular}{c|c|rrr|rrr|rrr|rrr|rrr}
    \toprule[1.2pt]
    \multirow{2}[2]{*}{\textbf{Subject}} & \multirow{2}[2]{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{I-Loops}} & \multicolumn{3}{c|}{\textbf{I-Latency(CPU)}} & \multicolumn{3}{c|}{\textbf{I-Energy(CPU)}} & \multicolumn{3}{c|}{\textbf{I-Latency(GPU)}} & \multicolumn{3}{c}{\textbf{I-Energy(GPU)}} \\
          &       & \multicolumn{1}{c}{\textbf{$\epsilon$ = 1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =3 }} \\
    \midrule
    \multirow{7}[2]{*}{\textbf{H-NLP}} & \textbf{Seq2Sick} & 4.31  & 5.84  & 12.28  & 4.83  & 8.85  & 19.55  & 4.84  & 8.85  & 21.47  & 3.73  & 5.90  & 13.24  & 3.77  & 5.96  & 13.33  \\
          & \textbf{SynError} & 19.09  & 19.59  & 19.59  & 19.35  & 19.82  & 19.82  & 19.63  & 20.10  & 20.10  & 14.14  & 14.52  & 14.52  & 14.27  & 14.65  & 14.65  \\
          & \textbf{SIT} & 11.83  & 5.99  & 5.35  & -1.68  & -8.53  & -11.21  & 8.17  & 6.32  & 7.41  & 9.84  & 5.50  & 5.75  & 9.90  & 5.58  & 5.83  \\
          & \textbf{TransRepair} & 0.17  & 0.17  & 0.17  & 0.76  & 0.10  & 0.10  & 0.93  & 0.33  & 0.33  & -0.07  & 0.00  & 0.00  & -0.07  & 0.00  & 0.00  \\
          & \textbf{\tool(C)} & 564.45  & 995.45  & 1357.77  & 764.92  & 1487.92  & 2015.70  & 785.60  & 1471.26  & 1967.05  & 462.24  & 851.80  & 1116.80  & 406.39  & 755.18  & 972.92  \\
          & \textbf{\tool(T)} & 2697.77  & 3735.38  & 3917.91  & 3153.97  & 4481.93  & 4681.28  & 3052.62  & 4544.65  & 4759.71  & 1953.57  & 2729.83  & 2854.89  & 1532.91  & 2137.53  & 2221.66  \\
          & \textbf{\tool(S)} & 142.31  & 311.06  & 612.08  & 146.51  & 451.93  & 877.79  & 147.70  & 461.30  & 870.72  & 101.21  & 275.58  & 523.04  & 95.05  & 259.88  & 508.80  \\
    \midrule
    \multirow{7}[2]{*}{\textbf{AllenAI}} & \textbf{Seq2Sick} & 1.72  & 2.22  & 2.15  & 1.48  & 2.06  & 1.35  & 1.19  & 1.76  & 1.10  & 1.57  & 1.41  & 0.38  & 1.70  & 1.57  & 0.57  \\
          & \textbf{SynError} & 0.38  & 0.38  & 0.38  & 1.89  & 1.89  & 1.89  & 1.75  & 1.75  & 1.75  & -0.85  & -0.85  & -0.85  & -0.71  & -0.71  & -0.71  \\
          & \textbf{SIT} & 7.06  & 4.12  & 6.67  & 1.73  & -3.24  & -4.64  & 1.73  & -3.24  & -4.60  & 3.95  & 14.25  & -2.05  & 4.12  & 14.64  & -1.60  \\
          & \textbf{TransRepair} & 0.08  & 0.08  & 0.08  & -0.37  & -0.37  & -0.37  & -0.55  & -0.55  & -0.55  & -0.15  & -0.15  & -0.15  & -0.14  & -0.14  & -0.14  \\
          & \textbf{\tool(C)} & 35.16  & 74.90  & 103.36  & 26.69  & 45.77  & 85.09  & 27.48  & 48.09  & 86.00  & 21.82  & 35.43  & 91.48  & 22.12  & 43.21  & 98.46  \\
          & \textbf{\tool(T)} & 24.83  & 42.04  & 56.75  & 49.12  & 62.84  & 67.98  & 49.99  & 62.65  & 69.06  & 30.65  & 41.32  & 46.09  & 31.00  & 41.81  & 49.66  \\
          & \textbf{\tool(S)} & 66.21  & 108.67  & 128.60  & 86.05  & 139.03  & 164.57  & 84.17  & 135.71  & 160.95  & 69.57  & 112.88  & 132.68  & 68.79  & 115.23  & 137.06  \\
    \midrule
    \multirow{7}[2]{*}{\textbf{T5}} & \textbf{Seq2Sick} & 7.09  & 6.28  & -6.03  & 7.21  & 6.04  & -5.97  & 8.55  & 6.88  & -5.16  & 9.01  & 8.00  & -3.97  & 8.85  & 16.94  & 4.50  \\
          & \textbf{SynError} & 2.18  & 2.18  & 2.18  & 3.20  & 3.20  & 3.20  & 2.11  & 2.11  & 2.11  & 1.02  & 1.02  & 1.02  & 1.13  & 1.13  & 1.13  \\
          & \textbf{SIT} & -8.06  & 1.05  & 6.27  & -4.51  & 7.79  & 7.38  & -3.79  & 9.84  & 10.59  & -10.99  & 3.57  & 7.74  & -10.90  & 3.78  & 8.07  \\
          & \textbf{TransRepair} & 3.73  & 8.06  & 8.06  & 4.90  & 9.47  & 9.26  & 6.42  & 11.39  & 10.74  & 3.70  & 8.34  & 8.35  & 3.76  & 8.42  & 8.39  \\
          & \textbf{\tool(C)} & 168.92  & 198.36  & 205.37  & 191.05  & 225.48  & 233.01  & 194.45  & 228.02  & 234.04  & 164.61  & 194.79  & 202.28  & 165.38  & 195.77  & 203.29  \\
          & \textbf{\tool(T)} & 307.27  & 328.94  & 328.94  & 352.14  & 376.55  & 376.55  & 347.74  & 373.85  & 373.85  & 305.37  & 325.61  & 325.61  & 331.85  & 352.25  & 352.25  \\
          & \textbf{\tool(S)} & 77.67  & 80.56  & 82.52  & 85.72  & 89.11  & 91.38  & 86.90  & 90.29  & 92.56  & 75.77  & 78.68  & 80.66  & 68.79  & 73.03  & 74.56  \\
    \bottomrule[1.2pt]
    \end{tabular}%
    }
  \label{tab:severity}%
\end{table*}%



==> Table/severity_B.tex <==
% Table generated by Excel2LaTeX from sheet 'Effectiveness'
% Table generated by Excel2LaTeX from sheet 'Effectiveness'

\begin{table*}[tp]
  \centering
  \caption{The Effectiveness Results of \textcolor{blue}{\tool-B} in Degrading \textcolor{blue}{LLMs} Performance}
  \resizebox{0.98\textwidth}{!}{
        \begin{tabular}{c|c|rrr|rrr|rrr|rrr|rrr}
    \toprule[1.2pt]
    \multirow{2}[2]{*}{\textbf{Subject}} & \multirow{2}[2]{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{I-Loops}} & \multicolumn{3}{c|}{\textbf{I-Latency(CPU)}} & \multicolumn{3}{c|}{\textbf{I-Energy(CPU)}} & \multicolumn{3}{c|}{\textbf{I-Latency(GPU)}} & \multicolumn{3}{c}{\textbf{I-Energy(GPU)}} \\
          &       & \multicolumn{1}{c}{\textbf{$\epsilon$ = 1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c|}{\textbf{$\epsilon$ =3 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =1 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =2 }} & \multicolumn{1}{c}{\textbf{$\epsilon$ =3 }} \\
\midrule
\multirow{3}[1]{*}{\textbf{H-NLP}} & \textbf{\tool/B (C)} & 907.89 & 1,483.58 & 2,032.41 & 815.15 & 1,561.45 & 2,139.55 & 1,026.17 & 1,948.84 & 2,653.57 & 684.34 & 1,330.43 & 1,823.64 & 681.23 & 1,326.60 & 1,821.57 \\
      & \textbf{\tool/B (T)} & 2,556.56 & 3,064.19 & 3,043.95 & 2,557.49 & 3,099.16 & 2,996.62 & 3,106.02 & 3,807.87 & 3,700.27 & 1,968.85 & 2,451.50 & 2,416.83 & 1,965.72 & 2,451.54 & 2,419.52 \\
      & \textbf{\tool/B (S)} & 200.15 & 450.31 & 809.79 & 181.05 & 389.76 & 766.62 & 233.63 & 488.25 & 973.90 & 172.32 & 369.99 & 683.68 & 172.01 & 369.75 & 683.28 \\
\midrule
\multirow{3}[1]{*}{\textbf{AllenAI}} & \textbf{\tool/B (C)} & 31.78 & 84.30 & 116.75 & 225.80 & 935.84 & 143.91 & 43.25 & 132.30 & 194.46 & 27.64 & 97.85 & 148.22 & 27.41 & 97.47 & 147.72 \\
      & \textbf{\tool/B (T)} & 71.37 & 131.54 & 121.88 & 56.40 & 119.95 & 146.99 & 85.25 & 163.81 & 196.13 & 60.21 & 123.44 & 152.83 & 59.93 & 123.10 & 152.54 \\
      & \textbf{\tool/B (S)} & 65.82 & 76.05 & 90.41 & 78.24 & 90.00 & 80.83 & 110.20 & 123.05 & 113.93 & 80.90 & 92.03 & 86.14 & 80.57 & 91.73 & 85.87 \\
\midrule
\multirow{3}[1]{*}{\textbf{T5}} & \textbf{\tool/B (C)} & 231.95 & 255.70 & 259.05 & 239.17 & 257.96 & 259.95 & 279.77 & 303.05 & 305.42 & 233.26 & 257.03 & 261.46 & 233.86 & 257.69 & 262.09 \\
      & \textbf{\tool/B (T)} & 318.94 & 293.67 & 257.92 & 331.77 & 304.63 & 272.73 & 384.44 & 350.53 & 311.98 & 319.07 & 294.36 & 259.99 & 319.65 & 294.84 & 260.43 \\
      & \textbf{\tool/B (S)} & 252.44 & 279.53 & 289.54 & 260.69 & 288.66 & 295.31 & 300.39 & 333.39 & 341.33 & 252.44 & 279.23 & 288.46 & 252.48 & 279.22 & 288.41 \\
\midrule
\multirow{3}[1]{*}{\textbf{U-DL}} & \textbf{\tool/B (C)} & 488.81 & 495.81 & 502.85 & 522.33 & 517.47 & 526.17 & 559.45 & 556.72 & 567.10 & 483.54 & 490.87 & 499.09 & 483.52 & 490.88 & 499.15 \\
      & \textbf{\tool/B (T)} & 502.85 & 502.85 & 494.97 & 536.77 & 527.40 & 511.22 & 579.50 & 570.67 & 557.33 & 498.65 & 499.99 & 496.64 & 498.56 & 499.90 & 496.46 \\
      & \textbf{\tool/B (S)} & 466.97 & 490.19 & 501.44 & 507.14 & 517.67 & 525.86 & 541.40 & 558.12 & 567.17 & 463.23 & 490.47 & 511.64 & 463.31 & 490.69 & 511.80 \\
\midrule
\multirow{3}[1]{*}{\textbf{FairSeq}} & \textbf{\tool/B (C)} & 33.09 & 43.60 & 72.18 & 26.76 & 34.61 & 69.78 & 31.94 & 40.82 & 79.01 & 29.29 & 39.99 & 76.06 & 29.36 & 40.19 & 76.36 \\
      & \textbf{\tool/B (T)} & 41.71 & 66.82 & 87.19 & 32.97 & 58.12 & 75.42 & 39.15 & 66.41 & 85.81 & 36.04 & 64.10 & 85.87 & 36.10 & 64.18 & 85.95 \\
      & \textbf{\tool/B (S)} & 19.04 & 31.29 & 38.51 & 12.24 & 20.73 & 26.06 & 16.94 & 26.55 & 32.40 & 15.71 & 26.25 & 32.80 & 15.72 & 26.29 & 32.85 \\
\midrule
\multirow{3}[1]{*}{\textbf{MarianMT}} & \textbf{\tool/B (C)} & 65.70 & 185.56 & 264.37 & 55.72 & 173.09 & 298.05 & 67.01 & 200.74 & 338.54 & 55.62 & 164.33 & 282.05 & 55.46 & 163.84 & 282.20 \\
      & \textbf{\tool/B (T)} & 223.05 & 517.87 & 722.71 & 229.07 & 580.01 & 752.90 & 260.24 & 660.71 & 860.89 & 199.48 & 508.85 & 674.54 & 199.44 & 509.79 & 675.87 \\
      & \textbf{\tool/B (S)} & 42.43 & 68.25 & 78.04 & 35.36 & 64.01 & 65.18 & 44.70 & 77.00 & 78.26 & 36.10 & 64.71 & 69.38 & 36.06 & 64.67 & 69.41 \\
\midrule
\multirow{3}[1]{*}{\textbf{Flan-T5}} & \textbf{\tool/B (C)} & 421.97 & 628.14 & 850.14 & 426.32 & 629.20 & 845.69 & 495.38 & 726.82 & 980.89 & 426.82 & 637.66 & 897.14 & 426.87 & 638.74 & 868.34 \\
      & \textbf{\tool/B (T)} & 1,242.18 & 1,338.54 & 1,341.69 & 1,240.60 & 1,333.61 & 1,322.22 & 1,422.94 & 1,543.97 & 1,533.38 & 1,256.64 & 1,378.93 & 1,389.51 & 1,258.92 & 1,381.33 & 1,391.86 \\
      & \textbf{\tool/B (S)} & 572.45 & 892.17 & 1,082.76 & 564.03 & 879.97 & 1,064.21 & 652.28 & 1,015.91 & 1,235.05 & 567.71 & 884.32 & 1,076.55 & 568.44 & 885.57 & 1,077.70 \\
\midrule
\multirow{3}[1]{*}{\textbf{LaMini-GPT}} & \textbf{\tool/B (C)} & 140.67 & 208.14 & 240.05 & 764.30 & 1,109.99 & 1,211.88 & 943.59 & 1,385.40 & 1,525.22 & 733.99 & 1,111.11 & 1,260.97 & 734.45 & 1,112.28 & 1,263.29 \\
      & \textbf{\tool/B (T)} & 242.05 & 232.44 & 246.41 & 1,225.62 & 1,129.45 & 1,223.03 & 1,510.56 & 1,401.18 & 1,513.43 & 1,224.47 & 1,143.59 & 1,249.03 & 1,225.86 & 1,145.94 & 1,252.04 \\
      & \textbf{\tool/B (S)} & 191.80 & 208.14 & 225.11 & 998.56 & 1,069.81 & 1,127.94 & 1,222.32 & 1,328.29 & 1,407.41 & 962.31 & 1,051.01 & 1,138.46 & 962.76 & 1,052.40 & 1,140.30 \\
\midrule
\multirow{3}[1]{*}{\textbf{CodeGen}} & \textbf{\tool/B (C)} & 147.75 & 170.76 & 175.70 & 463.20 & 518.89 & 523.96 & 481.57 & 540.51 & 549.87 & 501.99 & 582.24 & 603.35 & 501.99 & 582.47 & 603.57 \\
      & \textbf{\tool/B (T)} & 118.40 & 154.85 & 146.01 & 378.35 & 496.82 & 451.94 & 394.97 & 517.96 & 475.82 & 405.33 & 551.65 & 528.71 & 405.63 & 552.12 & 529.16 \\
      & \textbf{\tool/B (S)} & 152.02 & 166.56 & 158.82 & 488.73 & 523.34 & 494.20 & 507.41 & 547.59 & 519.25 & 521.24 & 578.62 & 563.35 & 521.44 & 578.88 & 563.62 \\
    \bottomrule[1.2pt]
    \end{tabular}%
    }
  \label{tab:severity_B}%
\end{table*}%



==> Table/token.tex <==
% Table generated by Excel2LaTeX from sheet 'character'
\begin{table}[tbph]
  \centering
  \caption{The severity of token-level adversarial attacks}
  \resizebox{.49\textwidth}{!}{
            \begin{tabular}{c|c|cc|cc|cc}
    \toprule
    \multirow{2}[2]{*}{\textbf{NMT}} & \multirow{2}[2]{*}{\textbf{Perturbation}} & \multicolumn{2}{c|}{\textbf{I-FLOPs}} & \multicolumn{2}{c|}{\textbf{I-Latency    (CPU)}} & \multicolumn{2}{c}{\textbf{I-Latency    (GPU)}} \\
          &       & \textbf{Baseline} & \textbf{Ours} & \textbf{Baseline} & \textbf{Ours} & \textbf{Baseline} & \textbf{Ours} \\
    \midrule
    \multirow{5}[2]{*}{\textbf{H-NLP}} & \textbf{1} & 4.18  & \textbf{1318.72 } & 4.51  & \textbf{1485.64 } & 2.55  & \textbf{1269.53 } \\
          & \textbf{2} & 6.03  & \textbf{2131.92 } & 6.33  & \textbf{2403.21 } & 3.05  & \textbf{2054.83 } \\
          & \textbf{3} & 12.94  & \textbf{2336.88 } & 13.83  & \textbf{2636.51 } & 11.10  & \textbf{2296.09 } \\
          & \textbf{4} & 17.57  & \textbf{2360.94 } & 19.40  & \textbf{2664.46 } & 15.68  & \textbf{2314.23 } \\
          & \textbf{5} & 23.56  & \textbf{2366.09 } & 25.38  & \textbf{2669.82 } & 23.89  & \textbf{2321.93 } \\
    \midrule
    \multirow{5}[2]{*}{\textbf{FairSeq}} & \textbf{1} & -0.05  & \textbf{23.46 } & 0.15  & \textbf{24.85 } & 3.50  & \textbf{29.62 } \\
          & \textbf{2} & -0.19  & \textbf{36.80 } & 0.61  & \textbf{38.97 } & 1.17  & \textbf{40.59 } \\
          & \textbf{3} & -2.22  & \textbf{47.27 } & -0.73  & \textbf{51.21 } & -1.40  & \textbf{54.44 } \\
          & \textbf{4} & -5.78  & \textbf{57.60 } & -4.17  & \textbf{63.35 } & -4.09  & \textbf{63.57 } \\
          & \textbf{5} & -8.20  & \textbf{80.75 } & -6.85  & \textbf{89.73 } & -1.76  & \textbf{85.74 } \\
    \midrule
    \multirow{5}[2]{*}{\textbf{T5}} & \textbf{1} & 10.09  & \textbf{335.41 } & 9.66  & \textbf{383.38 } & 7.87  & \textbf{352.88 } \\
          & \textbf{2} & 6.80  & \textbf{343.69 } & 5.44  & \textbf{393.20 } & 4.06  & \textbf{362.45 } \\
          & \textbf{3} & 1.47  & \textbf{343.69 } & 1.64  & \textbf{393.20 } & -1.54  & \textbf{362.45 } \\
          & \textbf{4} & -11.66  & \textbf{343.69 } & -9.62  & \textbf{393.20 } & -8.28  & \textbf{362.45 } \\
          & \textbf{5} & -25.18  & \textbf{343.69 } & -24.29  & \textbf{393.20 } & -8.59  & \textbf{362.45 } \\
    \bottomrule
    \end{tabular}%
   }
  \label{tab:token_res}%
\end{table}%


==> Table/w_black.tex <==
% Table generated by Excel2LaTeX from sheet 'transfer'
\begin{table}[htbp]
  \centering
  \caption{The maximum I-FLOPs of blackbox token-level attack}
  \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{c|c|rrrrr}
    \toprule
    \textbf{Source} & \textbf{Target } & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{2}} & \multicolumn{1}{c}{\textbf{3}} & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{5}} \\
    \midrule
    \multirow{2}[2]{*}{\textbf{H-NLP}} & \textbf{FairSeq} & 185.71  & 57.14  & 68.75  & 57.14  & 42.86  \\
          & \textbf{T5} & 1600.00  & 1600.00  & 1600.00  & 1600.00  & 1600.00  \\
    \midrule
    \multirow{2}[2]{*}{\textbf{FairSeq}} & \textbf{H-NLP} & 6566.67  & 6566.67  & 6566.67  & 6566.67  & 6566.67  \\
          & \textbf{T5} & 1600.00  & 1600.00  & 1600.00  & 1600.00  & 1600.00  \\
    \midrule
    \multirow{2}[2]{*}{\textbf{T5}} & \textbf{H-NLP} & 3733.33  & 3733.33  & 3733.33  & 3733.33  & 3733.33  \\
          & \textbf{FairSeq} & 858.33  & 1816.67  & 1816.67  & 945.45  & 945.45  \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:w_black}%
\end{table}%


==> ablation.tex <==

\textcolor{red}{\section{ABLATION STUDY}}

\noindent\textcolor{red}{In this experiment, we carried out ablation studies to assess the efficacy of \(p_i^{o_i}\) in \tool for identifying critical tokens, as illustrated in \equref{eq:obj}.
The inspiration for this component came from recent research, which showed that the sequence of tokens output by a model also affects the generation of the EOS token \cite{DBLP:conf/blackboxnlp/NewmanHLM20,liu2022length,DBLP:conf/nips/AnilWALMRSGDN22}. To validate this idea's effectiveness for \tool and ensure it aligns with our overarching goals, we removed \(p_i^{o_i}\) in \equref{eq:obj} from the function \(f(x)\) and conducted the same attack execution operations.}

\input{Table/ablation}

\noindent\textcolor{red}{\fakeparagraph{Experimental Setup}
In our evaluation of various LLMs, we randomly chose 1,000 seed inputs
and applied \tool (with \(p_i^{o_i}\) removed from \(f(x)\)) to generate 1,000 abnormal inputs for each type of perturbation. The evaluation metrics employed adhere to those detailed in \secref{sec:severity}. Correspondingly, we averaged the experimental outcomes over three runs.}


\noindent\textcolor{red}{\fakeparagraph{Experimental Results} The results are shown in \tabref{tab:ablation}, providing a contrast with the results in \tabref{tab:severity_all}. From the results, we make two observations:
\textit{(i)}
The test samples generated in the ablation study exhibit a weaker degradation in computational efficiency for LLMs. Specifically, the required Loops, CPU latency, CPU energy consumption, GPU latency, and GPU energy consumption decreased on average by 14.88\%, 19.45\%, 13.82\%, 14.31\%, and 15.30\%, respectively.
\textit{(ii)} The decoder-only models are more sensitive to such components. Notably, during the ablation study, the GPU latency of LaMini-GPT saw a significant decrease of 74.07\% compared to control experiments. In contrast, models based on an encoder-decoder architecture exhibited a maximum reduction of only 45.83\%. This heightened sensitivity in decoder-only models can be attributed to their autoregressive nature, which makes them more susceptible to the influence of output context. Therefore, the results demonstrate the effectiveness of the 
\(p_i^{o_i}\) component in \tool for identifying critical tokens.}


==> config/packageref.tex <==
\usepackage{xcolor,colortbl}
\usepackage{graphicx}
\usepackage{color}
\usepackage{pifont}
\usepackage{ifthen}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage[inline]{enumitem}
\usepackage[ruled,linesnumbered]{algorithm2e}
\usepackage{tcolorbox}
\usepackage{booktabs}
\usepackage{tabularx}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}%
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}%
\newcolumntype{C}{>{\centering\arraybackslash}X}%
\usepackage{listings}
\lstset{
    breaklines=true,
    frame=lines,
    basicstyle=\ttfamily\scriptsize,
    keywordstyle=\color{purple}\bfseries,
    stringstyle=\color{brown},
    commentstyle=\color{teal},
    captionpos=b,
    xleftmargin=6pt,
    numbersep=3pt,
    numbers=left,
    tabsize=2,
}

\usepackage{relsize}
\usepackage{threeparttable}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{tikz}
% \usepackage{stackengine}
\usepackage{fontawesome}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{titlesec}
\usepackage{xspace}

\usepackage{gnuplottex}

% Workaround for bugs in lstlinebgrd
% From https://tex.stackexchange.com/questions/451532/recent-issues-with-lstlinebgrd-package-with-listings-after-the-latters-updates
% It works although I don't know why.
\usetikzlibrary{shapes,positioning}
\makeatletter
\let\old@lstKV@SwitchCases\lstKV@SwitchCases
\def\lstKV@SwitchCases#1#2#3{}
\makeatother
\usepackage{lstlinebgrd}
\makeatletter
\let\lstKV@SwitchCases\old@lstKV@SwitchCases

\lst@Key{numbers}{none}{%
    \def\lst@PlaceNumber{\lst@linebgrd}%
    \lstKV@SwitchCases{#1}%
    {none:\\%
        left:\def\lst@PlaceNumber{\llap{\normalfont
                \lst@numberstyle{\thelstnumber}\kern\lst@numbersep}\lst@linebgrd}\\%
        right:\def\lst@PlaceNumber{\rlap{\normalfont
                \kern\linewidth \kern\lst@numbersep
                \lst@numberstyle{\thelstnumber}}\lst@linebgrd}%
    }{\PackageError{Listings}{Numbers #1 unknown}\@ehc}}
\makeatother


==> config/topmatters.tex <==

\title{\tool: Automated Generation and Repair of Stub Code for Mock Objects}
\titlenote{This paper was accepted by the \emph{ACM Transactions on Software Engineering and Methodology} (TOSEM) in July 2023.}

\acmJournal{TOSEM}

\keywords{Software Testing, Mocking, Test Generation and Repair, Genetic Programming, Evolutionary Computation, Program Analysis}
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10011007.10011074.10011784</concept_id>
       <concept_desc>Software and its engineering~Search-based software engineering</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10011007.10011074.10011099.10011102.10011103</concept_id>
       <concept_desc>Software and its engineering~Software testing and debugging</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10011007.10011074.10011092.10011782</concept_id>
       <concept_desc>Software and its engineering~Automatic programming</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
   <concept>
       <concept_id>10011007.10011074.10011111.10011113</concept_id>
       <concept_desc>Software and its engineering~Software evolution</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Software and its engineering~Search-based software engineering}
\ccsdesc[500]{Software and its engineering~Software testing and debugging}
\ccsdesc[300]{Software and its engineering~Automatic programming}
\ccsdesc[300]{Software and its engineering~Software evolution}

\author{Hengcheng Zhu}
\orcid{0000-0002-3082-5957}
\email{hzhuaq@connect.ust.hk}
\affiliation{%
    \institution{The Hong Kong University of Science and Technology}
    \city{Hong Kong}
    \country{China}
}

\author{Lili Wei}
\orcid{0000-0002-2428-4111}
\email{lili.wei@mcgill.ca}
\affiliation{%
    \institution{McGill University}
    \city{Montreal}
    \country{Canada}
}

\author{Valerio Terragni}
\orcid{0000-0001-5885-9297}
\email{v.terragni@auckland.ac.nz}
\affiliation{%
    \institution{The University of Auckland}
    \city{Auckland}
    \country{New Zealand}
}

\author{Yepang Liu}
\orcid{0000-0001-8147-8126}
\email{liuyp1@sustech.edu.cn}
\affiliation{%
    \department{Department of Computer Science and Engineering}
    \department{Research Institute of Trustworthy Autonomous Systems}
    \institution{Southern University of Science and Technology}
    \city{Shenzhen}
    \country{China}
}

\author{Shing-Chi Cheung}
\authornote{Shing-Chi Cheung is the corresponding author.}
\orcid{0000-0002-3508-7172}
\email{scc@cse.ust.hk}
\affiliation{%
    \institution{The Hong Kong University of Science and Technology}
    \city{Hong Kong}
    \country{China}
}

\author{Jiarong Wu}
\orcid{0000-0001-6126-303X}
\email{jwubf@cse.ust.hk}
\affiliation{%
    \institution{The Hong Kong University of Science and Technology}
    \city{Hong Kong}
    \country{China}
}

\author{Qin Sheng}
\orcid{0009-0004-8527-9297}
\email{entersheng@webank.com}

\author{Bing Zhang}
\orcid{0009-0007-5862-136X}
\email{billzzhang@webank.com}

\author{Lihong Song}
\orcid{0009-0004-9452-4741}
\email{jeaninesong@webank.com}
\affiliation{%
    \institution{WeBank Co. Ltd.}
    \city{Shenzhen}
    \country{China}
}

% ACCORDING TO ACM STANDARDS we need to put et al. if the auhtors are more than two
\renewcommand{\shortauthors}{H. Zhu et al.}

\received{August 10, 2022}
\received[revised]{April 11, 2023}
\received[revised]{June 15, 2023}
\received[accepted]{July 23, 2023}


==> config/utilities.tex <==


\ifthenelse{\isundefined{\editmode}}{
\newcommand{\editnote}[3]{%
}
\newcommand{\updated}[1]{#1%
}
}{
\newcommand{\editnote}[3]{\xspace\colorbox{#1}{\sffamily \smaller \textcolor{white}{~\faCommenting{}~#2~}}\textcolor{#1}{~#3}\xspace}
\newcommand{\updated}[1]{\textcolor{violet}{#1}}
}

\definecolor{nord0}{HTML}{2E3440}
\definecolor{nord1}{HTML}{3B4252}
\definecolor{nord2}{HTML}{434C5E}
\definecolor{nord3}{HTML}{4C566A}
\definecolor{nord4}{HTML}{D8DEE9}
\definecolor{nord5}{HTML}{E5E9F0}
\definecolor{nord6}{HTML}{ECEFF4}
\definecolor{nord7}{HTML}{8FBCBB}
\definecolor{nord8}{HTML}{88C0D0}
\definecolor{nord9}{HTML}{81A1C1}
\definecolor{nord10}{HTML}{5E81AC}
\definecolor{nord11}{HTML}{BF616A}
\definecolor{nord12}{HTML}{D08770}
\definecolor{nord13}{HTML}{EBCB8B}
\definecolor{nord14}{HTML}{A3BE8C}
\definecolor{nord15}{HTML}{B48EAD}

\newcommand{\yepang}[1]{\editnote{nord11}{Yepang}{#1}}
\newcommand{\hc}[1]{\editnote{nord10}{HC}{#1}}
\newcommand{\scc}[1]{\editnote{purple}{SCC}{#1}}
\newcommand{\lili}[1]{\editnote{cyan}{Lili}{#1}}
\newcommand{\jr}[1]{\editnote{brown}{Jiarong}{#1}}
\newcommand{\valerio}[1]{\editnote{nord12}{Valerio}{#1}}

\newcommand{\tool}{\textsc{StubCoder}\@\xspace}
\newcommand{\mockito}{\textsc{Mockito}\@\xspace}
\newcommand{\easymock}{\textsc{EasyMock}\@\xspace}
\newcommand{\java}{\textsc{Java}\@\xspace}
\newcommand{\moq}{\textsc{Moq4}\@\xspace}
\newcommand{\junit}{\textsc{JUnit}\@\xspace}
\newcommand{\arja}{\textsc{Arja}\@\xspace}
\newcommand{\cardumen}{\textsc{Cardumen}\@\xspace}
\newcommand{\astor}{\textsc{Astor}\@\xspace}
\newcommand{\eg}[1]{(e.g., #1)}
\newcommand{\ie}[1]{(i.e., #1)}
\newcommand{\etal}[0]{et al.}

\newcommand{\numOfBenchmarkProjects}{13}
\newcommand{\numOfBenchmarkEntries}{59}
\newcommand{\testTuple}{\tau{} = \left\langle{} V, S, E, A\right\rangle}

\newcommand{\code}[1]{\text{\ttfamily#1}}

\definecolor{boxbg}{RGB}{240, 240 ,240}

\newenvironment{toberemoved}{%
\begin{tcolorbox}[title={To be Removed},boxrule=0.5pt,arc=0mm,colframe=red!50!white,colback=red!05!white]
}{\end{tcolorbox}}

\newcounter{rq}
\newenvironment{answertorq}{%
    \begin{tcolorbox}[
            arc=2mm,
            boxrule=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt
        ]
    \textbf{\faLightbulbO\ RQ\refstepcounter{rq}\therq{} in Summary:}
}{\end{tcolorbox}}

\tcbuselibrary{breakable}

\newenvironment{revised}{%
    \begin{tcolorbox}[
            arc=0mm,
            breakable,
            boxrule=0pt,
            left=4pt,
            right=4pt,
            top=4pt,
            bottom=4pt,
            % leftrule=1pt,
            % colback=nord14!15!white,
            % colframe=nord14,
        ]
}{\end{tcolorbox}}

\titleformat*{\paragraph}{\bfseries}



==> discussion.tex <==

\section{Discussion}

